Fairness in generative modeling

We design general-purpose algorithms for addressing fairness issues and mode collapse in generative modeling. More precisely, to design fair algorithms for as many sensitive variables as possible, including variables we might not be aware of, we assume no prior knowledge of sensitive variables: our algorithms use unsupervised fairness only, meaning no information related to the sensitive variables is used for our fairness-improving methods. All images of faces (even generated ones) have been removed to mitigate legal risks.

==> data_rw.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|c|}\\  Source & Target & Num. vars & Related side & Arity & Variable & Before fix & After fix (%
  CMA 0 &  CMA 10 & 80 & True & 2 & 111 & 0.507 & 86 \\ 
\end{tabular}
\begin{tabular}{|c|c|c|c|c|c|c|c|}\\  Source & Target & Num. vars & Related side & Arity & Variable & Before fix & After fix (%
  CMA 0 &  CMA 10 & 80 & True & 2 & 111 & 0.507 & 86 \\ 
 CMA 0 &  CMA 10 & 80 & True & 2 & 5 & 0.095 & 24 \\ 
\end{tabular}
\begin{tabular}{|c|c|c|c|c|c|c|c|}\\  Source & Target & Num. vars & Related side & Arity & Variable & Before fix & After fix (%
  CMA 0 &  CMA 10 & 80 & True & 2 & 111 & 0.507 & 86 \\ 
 CMA 0 &  CMA 10 & 80 & True & 2 & 5 & 0.095 & 24 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 111 & 0.622 & 84 \\ 
\end{tabular}
\begin{tabular}{|c|c|c|c|c|c|c|c|}\\  Source & Target & Num. vars & Related side & Arity & Variable & Before fix & After fix (%
  CMA 0 &  CMA 10 & 80 & True & 2 & 111 & 0.507 & 86 \\ 
 CMA 0 &  CMA 10 & 80 & True & 2 & 5 & 0.095 & 24 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 111 & 0.622 & 84 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 5 & 0.132 & 28 \\ 
\end{tabular}
\begin{tabular}{|c|c|c|c|c|c|c|c|}\\  Source & Target & Num. vars & Related side & Arity & Variable & Before fix & After fix (%
  CMA 0 &  CMA 10 & 80 & True & 2 & 111 & 0.507 & 86 \\ 
 CMA 0 &  CMA 10 & 80 & True & 2 & 5 & 0.095 & 24 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 111 & 0.622 & 84 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 5 & 0.132 & 28 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 111 & 0.729 & 82 \\ 
\end{tabular}
\begin{tabular}{|c|c|c|c|c|c|c|c|}\\  Source & Target & Num. vars & Related side & Arity & Variable & Before fix & After fix (%
  CMA 0 &  CMA 10 & 80 & True & 2 & 111 & 0.507 & 86 \\ 
 CMA 0 &  CMA 10 & 80 & True & 2 & 5 & 0.095 & 24 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 111 & 0.622 & 84 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 5 & 0.132 & 28 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 111 & 0.729 & 82 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 5 & 0.174 & 32 \\ 
\end{tabular}
\begin{tabular}{|c|c|c|c|c|c|c|c|}\\  Source & Target & Num. vars & Related side & Arity & Variable & Before fix & After fix (%
  CMA 0 &  CMA 10 & 80 & True & 2 & 111 & 0.507 & 86 \\ 
 CMA 0 &  CMA 10 & 80 & True & 2 & 5 & 0.095 & 24 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 111 & 0.622 & 84 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 5 & 0.132 & 28 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 111 & 0.729 & 82 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 5 & 0.174 & 32 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 111 & 0.09 & 97 \\ 
\end{tabular}
\begin{tabular}{|c|c|c|c|c|c|c|c|}\\  Source & Target & Num. vars & Related side & Arity & Variable & Before fix & After fix (%
  CMA 0 &  CMA 10 & 80 & True & 2 & 111 & 0.507 & 86 \\ 
 CMA 0 &  CMA 10 & 80 & True & 2 & 5 & 0.095 & 24 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 111 & 0.622 & 84 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 5 & 0.132 & 28 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 111 & 0.729 & 82 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 5 & 0.174 & 32 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 111 & 0.09 & 97 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 5 & 0.012 & 16 \\ 
\end{tabular}
\begin{tabular}{|c|c|c|c|c|c|c|c|}\\  Source & Target & Num. vars & Related side & Arity & Variable & Before fix & After fix (%
  CMA 0 &  CMA 10 & 80 & True & 2 & 111 & 0.507 & 86 \\ 
 CMA 0 &  CMA 10 & 80 & True & 2 & 5 & 0.095 & 24 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 111 & 0.622 & 84 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 5 & 0.132 & 28 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 111 & 0.729 & 82 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 5 & 0.174 & 32 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 111 & 0.09 & 97 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 5 & 0.012 & 16 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 111 & 0.146 & 88 \\ 
\end{tabular}
\begin{tabular}{|c|c|c|c|c|c|c|c|}\\  Source & Target & Num. vars & Related side & Arity & Variable & Before fix & After fix (%
  CMA 0 &  CMA 10 & 80 & True & 2 & 111 & 0.507 & 86 \\ 
 CMA 0 &  CMA 10 & 80 & True & 2 & 5 & 0.095 & 24 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 111 & 0.622 & 84 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 5 & 0.132 & 28 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 111 & 0.729 & 82 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 5 & 0.174 & 32 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 111 & 0.09 & 97 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 5 & 0.012 & 16 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 111 & 0.146 & 88 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 5 & 0.021 & 42 \\ 
\end{tabular}
\begin{tabular}{|c|c|c|c|c|c|c|c|}\\  Source & Target & Num. vars & Related side & Arity & Variable & Before fix & After fix (%
  CMA 0 &  CMA 10 & 80 & True & 2 & 111 & 0.507 & 86 \\ 
 CMA 0 &  CMA 10 & 80 & True & 2 & 5 & 0.095 & 24 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 111 & 0.622 & 84 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 5 & 0.132 & 28 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 111 & 0.729 & 82 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 5 & 0.174 & 32 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 111 & 0.09 & 97 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 5 & 0.012 & 16 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 111 & 0.146 & 88 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 5 & 0.021 & 42 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 111 & 0.232 & 93 \\ 
\end{tabular}
\begin{tabular}{|c|c|c|c|c|c|c|c|}\\  Source & Target & Num. vars & Related side & Arity & Variable & Before fix & After fix (%
  CMA 0 &  CMA 10 & 80 & True & 2 & 111 & 0.507 & 86 \\ 
 CMA 0 &  CMA 10 & 80 & True & 2 & 5 & 0.095 & 24 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 111 & 0.622 & 84 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 5 & 0.132 & 28 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 111 & 0.729 & 82 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 5 & 0.174 & 32 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 111 & 0.09 & 97 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 5 & 0.012 & 16 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 111 & 0.146 & 88 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 5 & 0.021 & 42 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 111 & 0.232 & 93 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 5 & 0.029 & 41 \\ 
\end{tabular}
\begin{tabular}{|c|c|c|c|c|c|c|c|}\\  Source & Target & Num. vars & Related side & Arity & Variable & Before fix & After fix (%
  CMA 0 &  CMA 10 & 80 & True & 2 & 111 & 0.507 & 86 \\ 
 CMA 0 &  CMA 10 & 80 & True & 2 & 5 & 0.095 & 24 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 111 & 0.622 & 84 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 5 & 0.132 & 28 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 111 & 0.729 & 82 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 5 & 0.174 & 32 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 111 & 0.09 & 97 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 5 & 0.012 & 16 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 111 & 0.146 & 88 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 5 & 0.021 & 42 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 111 & 0.232 & 93 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 5 & 0.029 & 41 \\ 
 origin &  CMA 10 & 80 & True & 2 & 5 & 0.231 & 29 \\ 
\end{tabular}
\begin{tabular}{|c|c|c|c|c|c|c|c|}\\  Source & Target & Num. vars & Related side & Arity & Variable & Before fix & After fix (%
  CMA 0 &  CMA 10 & 80 & True & 2 & 111 & 0.507 & 86 \\ 
 CMA 0 &  CMA 10 & 80 & True & 2 & 5 & 0.095 & 24 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 111 & 0.622 & 84 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 5 & 0.132 & 28 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 111 & 0.729 & 82 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 5 & 0.174 & 32 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 111 & 0.09 & 97 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 5 & 0.012 & 16 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 111 & 0.146 & 88 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 5 & 0.021 & 42 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 111 & 0.232 & 93 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 5 & 0.029 & 41 \\ 
 origin &  CMA 10 & 80 & True & 2 & 5 & 0.231 & 29 \\ 
 origin &  CMA 20 & 80 & True & 2 & 5 & 0.273 & 33 \\ 
\end{tabular}
\begin{tabular}{|c|c|c|c|c|c|c|c|}\\  Source & Target & Num. vars & Related side & Arity & Variable & Before fix & After fix (%
  CMA 0 &  CMA 10 & 80 & True & 2 & 111 & 0.507 & 86 \\ 
 CMA 0 &  CMA 10 & 80 & True & 2 & 5 & 0.095 & 24 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 111 & 0.622 & 84 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 5 & 0.132 & 28 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 111 & 0.729 & 82 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 5 & 0.174 & 32 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 111 & 0.09 & 97 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 5 & 0.012 & 16 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 111 & 0.146 & 88 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 5 & 0.021 & 42 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 111 & 0.232 & 93 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 5 & 0.029 & 41 \\ 
 origin &  CMA 10 & 80 & True & 2 & 5 & 0.231 & 29 \\ 
 origin &  CMA 20 & 80 & True & 2 & 5 & 0.273 & 33 \\ 
 origin &  CMA 40 & 80 & True & 2 & 5 & 0.321 & 40 \\ 
\end{tabular}
\begin{tabular}{|c|c|c|c|c|c|c|c|}\\  Source & Target & Num. vars & Related side & Arity & Variable & Before fix & After fix (%
  CMA 0 &  CMA 10 & 80 & True & 2 & 111 & 0.507 & 86 \\ 
 CMA 0 &  CMA 10 & 80 & True & 2 & 5 & 0.095 & 24 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 111 & 0.622 & 84 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 5 & 0.132 & 28 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 111 & 0.729 & 82 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 5 & 0.174 & 32 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 111 & 0.09 & 97 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 5 & 0.012 & 16 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 111 & 0.146 & 88 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 5 & 0.021 & 42 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 111 & 0.232 & 93 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 5 & 0.029 & 41 \\ 
 origin &  CMA 10 & 80 & True & 2 & 5 & 0.231 & 29 \\ 
 origin &  CMA 20 & 80 & True & 2 & 5 & 0.273 & 33 \\ 
 origin &  CMA 40 & 80 & True & 2 & 5 & 0.321 & 40 \\ 
 origin &  D1+1 10 & 80 & True & 2 & 5 & 0.142 & 30 \\ 
\end{tabular}
\begin{tabular}{|c|c|c|c|c|c|c|c|}\\  Source & Target & Num. vars & Related side & Arity & Variable & Before fix & After fix (%
  CMA 0 &  CMA 10 & 80 & True & 2 & 111 & 0.507 & 86 \\ 
 CMA 0 &  CMA 10 & 80 & True & 2 & 5 & 0.095 & 24 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 111 & 0.622 & 84 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 5 & 0.132 & 28 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 111 & 0.729 & 82 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 5 & 0.174 & 32 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 111 & 0.09 & 97 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 5 & 0.012 & 16 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 111 & 0.146 & 88 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 5 & 0.021 & 42 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 111 & 0.232 & 93 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 5 & 0.029 & 41 \\ 
 origin &  CMA 10 & 80 & True & 2 & 5 & 0.231 & 29 \\ 
 origin &  CMA 20 & 80 & True & 2 & 5 & 0.273 & 33 \\ 
 origin &  CMA 40 & 80 & True & 2 & 5 & 0.321 & 40 \\ 
 origin &  D1+1 10 & 80 & True & 2 & 5 & 0.142 & 30 \\ 
 origin &  D1+1 20 & 80 & True & 2 & 5 & 0.152 & 32 \\ 
\end{tabular}
\begin{tabular}{|c|c|c|c|c|c|c|c|}\\  Source & Target & Num. vars & Related side & Arity & Variable & Before fix & After fix (%
  CMA 0 &  CMA 10 & 80 & True & 2 & 111 & 0.507 & 86 \\ 
 CMA 0 &  CMA 10 & 80 & True & 2 & 5 & 0.095 & 24 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 111 & 0.622 & 84 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 5 & 0.132 & 28 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 111 & 0.729 & 82 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 5 & 0.174 & 32 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 111 & 0.09 & 97 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 5 & 0.012 & 16 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 111 & 0.146 & 88 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 5 & 0.021 & 42 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 111 & 0.232 & 93 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 5 & 0.029 & 41 \\ 
 origin &  CMA 10 & 80 & True & 2 & 5 & 0.231 & 29 \\ 
 origin &  CMA 20 & 80 & True & 2 & 5 & 0.273 & 33 \\ 
 origin &  CMA 40 & 80 & True & 2 & 5 & 0.321 & 40 \\ 
 origin &  D1+1 10 & 80 & True & 2 & 5 & 0.142 & 30 \\ 
 origin &  D1+1 20 & 80 & True & 2 & 5 & 0.152 & 32 \\ 
 origin &  D1+1 40 & 80 & True & 2 & 5 & 0.16 & 26 \\ 
\end{tabular}
\begin{tabular}{|c|c|c|c|c|c|c|c|}\\  Source & Target & Num. vars & Related side & Arity & Variable & Before fix & After fix (%
  CMA 0 &  CMA 10 & 80 & True & 2 & 111 & 0.507 & 86 \\ 
 CMA 0 &  CMA 10 & 80 & True & 2 & 5 & 0.095 & 24 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 111 & 0.622 & 84 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 5 & 0.132 & 28 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 111 & 0.729 & 82 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 5 & 0.174 & 32 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 111 & 0.09 & 97 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 5 & 0.012 & 16 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 111 & 0.146 & 88 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 5 & 0.021 & 42 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 111 & 0.232 & 93 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 5 & 0.029 & 41 \\ 
 origin &  CMA 10 & 80 & True & 2 & 5 & 0.231 & 29 \\ 
 origin &  CMA 20 & 80 & True & 2 & 5 & 0.273 & 33 \\ 
 origin &  CMA 40 & 80 & True & 2 & 5 & 0.321 & 40 \\ 
 origin &  D1+1 10 & 80 & True & 2 & 5 & 0.142 & 30 \\ 
 origin &  D1+1 20 & 80 & True & 2 & 5 & 0.152 & 32 \\ 
 origin &  D1+1 40 & 80 & True & 2 & 5 & 0.16 & 26 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 111 & 0.507 & 99 \\ 
\end{tabular}
\begin{tabular}{|c|c|c|c|c|c|c|c|}\\  Source & Target & Num. vars & Related side & Arity & Variable & Before fix & After fix (%
  CMA 0 &  CMA 10 & 80 & True & 2 & 111 & 0.507 & 86 \\ 
 CMA 0 &  CMA 10 & 80 & True & 2 & 5 & 0.095 & 24 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 111 & 0.622 & 84 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 5 & 0.132 & 28 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 111 & 0.729 & 82 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 5 & 0.174 & 32 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 111 & 0.09 & 97 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 5 & 0.012 & 16 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 111 & 0.146 & 88 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 5 & 0.021 & 42 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 111 & 0.232 & 93 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 5 & 0.029 & 41 \\ 
 origin &  CMA 10 & 80 & True & 2 & 5 & 0.231 & 29 \\ 
 origin &  CMA 20 & 80 & True & 2 & 5 & 0.273 & 33 \\ 
 origin &  CMA 40 & 80 & True & 2 & 5 & 0.321 & 40 \\ 
 origin &  D1+1 10 & 80 & True & 2 & 5 & 0.142 & 30 \\ 
 origin &  D1+1 20 & 80 & True & 2 & 5 & 0.152 & 32 \\ 
 origin &  D1+1 40 & 80 & True & 2 & 5 & 0.16 & 26 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 111 & 0.507 & 99 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 5 & 0.095 & 92 \\ 
\end{tabular}
\begin{tabular}{|c|c|c|c|c|c|c|c|}\\  Source & Target & Num. vars & Related side & Arity & Variable & Before fix & After fix (%
  CMA 0 &  CMA 10 & 80 & True & 2 & 111 & 0.507 & 86 \\ 
 CMA 0 &  CMA 10 & 80 & True & 2 & 5 & 0.095 & 24 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 111 & 0.622 & 84 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 5 & 0.132 & 28 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 111 & 0.729 & 82 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 5 & 0.174 & 32 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 111 & 0.09 & 97 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 5 & 0.012 & 16 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 111 & 0.146 & 88 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 5 & 0.021 & 42 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 111 & 0.232 & 93 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 5 & 0.029 & 41 \\ 
 origin &  CMA 10 & 80 & True & 2 & 5 & 0.231 & 29 \\ 
 origin &  CMA 20 & 80 & True & 2 & 5 & 0.273 & 33 \\ 
 origin &  CMA 40 & 80 & True & 2 & 5 & 0.321 & 40 \\ 
 origin &  D1+1 10 & 80 & True & 2 & 5 & 0.142 & 30 \\ 
 origin &  D1+1 20 & 80 & True & 2 & 5 & 0.152 & 32 \\ 
 origin &  D1+1 40 & 80 & True & 2 & 5 & 0.16 & 26 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 111 & 0.507 & 99 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 5 & 0.095 & 92 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 111 & 0.622 & 100 \\ 
\end{tabular}
\begin{tabular}{|c|c|c|c|c|c|c|c|}\\  Source & Target & Num. vars & Related side & Arity & Variable & Before fix & After fix (%
  CMA 0 &  CMA 10 & 80 & True & 2 & 111 & 0.507 & 86 \\ 
 CMA 0 &  CMA 10 & 80 & True & 2 & 5 & 0.095 & 24 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 111 & 0.622 & 84 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 5 & 0.132 & 28 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 111 & 0.729 & 82 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 5 & 0.174 & 32 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 111 & 0.09 & 97 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 5 & 0.012 & 16 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 111 & 0.146 & 88 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 5 & 0.021 & 42 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 111 & 0.232 & 93 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 5 & 0.029 & 41 \\ 
 origin &  CMA 10 & 80 & True & 2 & 5 & 0.231 & 29 \\ 
 origin &  CMA 20 & 80 & True & 2 & 5 & 0.273 & 33 \\ 
 origin &  CMA 40 & 80 & True & 2 & 5 & 0.321 & 40 \\ 
 origin &  D1+1 10 & 80 & True & 2 & 5 & 0.142 & 30 \\ 
 origin &  D1+1 20 & 80 & True & 2 & 5 & 0.152 & 32 \\ 
 origin &  D1+1 40 & 80 & True & 2 & 5 & 0.16 & 26 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 111 & 0.507 & 99 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 5 & 0.095 & 92 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 111 & 0.622 & 100 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 5 & 0.132 & 97 \\ 
\end{tabular}
\begin{tabular}{|c|c|c|c|c|c|c|c|}\\  Source & Target & Num. vars & Related side & Arity & Variable & Before fix & After fix (%
  CMA 0 &  CMA 10 & 80 & True & 2 & 111 & 0.507 & 86 \\ 
 CMA 0 &  CMA 10 & 80 & True & 2 & 5 & 0.095 & 24 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 111 & 0.622 & 84 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 5 & 0.132 & 28 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 111 & 0.729 & 82 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 5 & 0.174 & 32 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 111 & 0.09 & 97 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 5 & 0.012 & 16 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 111 & 0.146 & 88 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 5 & 0.021 & 42 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 111 & 0.232 & 93 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 5 & 0.029 & 41 \\ 
 origin &  CMA 10 & 80 & True & 2 & 5 & 0.231 & 29 \\ 
 origin &  CMA 20 & 80 & True & 2 & 5 & 0.273 & 33 \\ 
 origin &  CMA 40 & 80 & True & 2 & 5 & 0.321 & 40 \\ 
 origin &  D1+1 10 & 80 & True & 2 & 5 & 0.142 & 30 \\ 
 origin &  D1+1 20 & 80 & True & 2 & 5 & 0.152 & 32 \\ 
 origin &  D1+1 40 & 80 & True & 2 & 5 & 0.16 & 26 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 111 & 0.507 & 99 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 5 & 0.095 & 92 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 111 & 0.622 & 100 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 5 & 0.132 & 97 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 111 & 0.729 & 99 \\ 
\end{tabular}
\begin{tabular}{|c|c|c|c|c|c|c|c|}\\  Source & Target & Num. vars & Related side & Arity & Variable & Before fix & After fix (%
  CMA 0 &  CMA 10 & 80 & True & 2 & 111 & 0.507 & 86 \\ 
 CMA 0 &  CMA 10 & 80 & True & 2 & 5 & 0.095 & 24 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 111 & 0.622 & 84 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 5 & 0.132 & 28 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 111 & 0.729 & 82 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 5 & 0.174 & 32 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 111 & 0.09 & 97 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 5 & 0.012 & 16 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 111 & 0.146 & 88 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 5 & 0.021 & 42 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 111 & 0.232 & 93 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 5 & 0.029 & 41 \\ 
 origin &  CMA 10 & 80 & True & 2 & 5 & 0.231 & 29 \\ 
 origin &  CMA 20 & 80 & True & 2 & 5 & 0.273 & 33 \\ 
 origin &  CMA 40 & 80 & True & 2 & 5 & 0.321 & 40 \\ 
 origin &  D1+1 10 & 80 & True & 2 & 5 & 0.142 & 30 \\ 
 origin &  D1+1 20 & 80 & True & 2 & 5 & 0.152 & 32 \\ 
 origin &  D1+1 40 & 80 & True & 2 & 5 & 0.16 & 26 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 111 & 0.507 & 99 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 5 & 0.095 & 92 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 111 & 0.622 & 100 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 5 & 0.132 & 97 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 111 & 0.729 & 99 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 5 & 0.174 & 100 \\ 
\end{tabular}
\begin{tabular}{|c|c|c|c|c|c|c|c|}\\  Source & Target & Num. vars & Related side & Arity & Variable & Before fix & After fix (%
  CMA 0 &  CMA 10 & 80 & True & 2 & 111 & 0.507 & 86 \\ 
 CMA 0 &  CMA 10 & 80 & True & 2 & 5 & 0.095 & 24 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 111 & 0.622 & 84 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 5 & 0.132 & 28 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 111 & 0.729 & 82 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 5 & 0.174 & 32 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 111 & 0.09 & 97 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 5 & 0.012 & 16 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 111 & 0.146 & 88 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 5 & 0.021 & 42 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 111 & 0.232 & 93 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 5 & 0.029 & 41 \\ 
 origin &  CMA 10 & 80 & True & 2 & 5 & 0.231 & 29 \\ 
 origin &  CMA 20 & 80 & True & 2 & 5 & 0.273 & 33 \\ 
 origin &  CMA 40 & 80 & True & 2 & 5 & 0.321 & 40 \\ 
 origin &  D1+1 10 & 80 & True & 2 & 5 & 0.142 & 30 \\ 
 origin &  D1+1 20 & 80 & True & 2 & 5 & 0.152 & 32 \\ 
 origin &  D1+1 40 & 80 & True & 2 & 5 & 0.16 & 26 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 111 & 0.507 & 99 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 5 & 0.095 & 92 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 111 & 0.622 & 100 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 5 & 0.132 & 97 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 111 & 0.729 & 99 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 5 & 0.174 & 100 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 2 & 111 & 0.09 & 128 \\ 
\end{tabular}
\begin{tabular}{|c|c|c|c|c|c|c|c|}\\  Source & Target & Num. vars & Related side & Arity & Variable & Before fix & After fix (%
  CMA 0 &  CMA 10 & 80 & True & 2 & 111 & 0.507 & 86 \\ 
 CMA 0 &  CMA 10 & 80 & True & 2 & 5 & 0.095 & 24 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 111 & 0.622 & 84 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 5 & 0.132 & 28 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 111 & 0.729 & 82 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 5 & 0.174 & 32 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 111 & 0.09 & 97 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 5 & 0.012 & 16 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 111 & 0.146 & 88 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 5 & 0.021 & 42 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 111 & 0.232 & 93 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 5 & 0.029 & 41 \\ 
 origin &  CMA 10 & 80 & True & 2 & 5 & 0.231 & 29 \\ 
 origin &  CMA 20 & 80 & True & 2 & 5 & 0.273 & 33 \\ 
 origin &  CMA 40 & 80 & True & 2 & 5 & 0.321 & 40 \\ 
 origin &  D1+1 10 & 80 & True & 2 & 5 & 0.142 & 30 \\ 
 origin &  D1+1 20 & 80 & True & 2 & 5 & 0.152 & 32 \\ 
 origin &  D1+1 40 & 80 & True & 2 & 5 & 0.16 & 26 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 111 & 0.507 & 99 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 5 & 0.095 & 92 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 111 & 0.622 & 100 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 5 & 0.132 & 97 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 111 & 0.729 & 99 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 5 & 0.174 & 100 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 2 & 111 & 0.09 & 128 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 2 & 5 & 0.012 & 41 \\ 
\end{tabular}
\begin{tabular}{|c|c|c|c|c|c|c|c|}\\  Source & Target & Num. vars & Related side & Arity & Variable & Before fix & After fix (%
  CMA 0 &  CMA 10 & 80 & True & 2 & 111 & 0.507 & 86 \\ 
 CMA 0 &  CMA 10 & 80 & True & 2 & 5 & 0.095 & 24 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 111 & 0.622 & 84 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 5 & 0.132 & 28 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 111 & 0.729 & 82 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 5 & 0.174 & 32 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 111 & 0.09 & 97 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 5 & 0.012 & 16 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 111 & 0.146 & 88 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 5 & 0.021 & 42 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 111 & 0.232 & 93 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 5 & 0.029 & 41 \\ 
 origin &  CMA 10 & 80 & True & 2 & 5 & 0.231 & 29 \\ 
 origin &  CMA 20 & 80 & True & 2 & 5 & 0.273 & 33 \\ 
 origin &  CMA 40 & 80 & True & 2 & 5 & 0.321 & 40 \\ 
 origin &  D1+1 10 & 80 & True & 2 & 5 & 0.142 & 30 \\ 
 origin &  D1+1 20 & 80 & True & 2 & 5 & 0.152 & 32 \\ 
 origin &  D1+1 40 & 80 & True & 2 & 5 & 0.16 & 26 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 111 & 0.507 & 99 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 5 & 0.095 & 92 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 111 & 0.622 & 100 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 5 & 0.132 & 97 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 111 & 0.729 & 99 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 5 & 0.174 & 100 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 2 & 111 & 0.09 & 128 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 2 & 5 & 0.012 & 41 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 2 & 111 & 0.146 & 98 \\ 
\end{tabular}
\begin{tabular}{|c|c|c|c|c|c|c|c|}\\  Source & Target & Num. vars & Related side & Arity & Variable & Before fix & After fix (%
  CMA 0 &  CMA 10 & 80 & True & 2 & 111 & 0.507 & 86 \\ 
 CMA 0 &  CMA 10 & 80 & True & 2 & 5 & 0.095 & 24 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 111 & 0.622 & 84 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 5 & 0.132 & 28 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 111 & 0.729 & 82 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 5 & 0.174 & 32 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 111 & 0.09 & 97 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 5 & 0.012 & 16 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 111 & 0.146 & 88 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 5 & 0.021 & 42 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 111 & 0.232 & 93 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 5 & 0.029 & 41 \\ 
 origin &  CMA 10 & 80 & True & 2 & 5 & 0.231 & 29 \\ 
 origin &  CMA 20 & 80 & True & 2 & 5 & 0.273 & 33 \\ 
 origin &  CMA 40 & 80 & True & 2 & 5 & 0.321 & 40 \\ 
 origin &  D1+1 10 & 80 & True & 2 & 5 & 0.142 & 30 \\ 
 origin &  D1+1 20 & 80 & True & 2 & 5 & 0.152 & 32 \\ 
 origin &  D1+1 40 & 80 & True & 2 & 5 & 0.16 & 26 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 111 & 0.507 & 99 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 5 & 0.095 & 92 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 111 & 0.622 & 100 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 5 & 0.132 & 97 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 111 & 0.729 & 99 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 5 & 0.174 & 100 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 2 & 111 & 0.09 & 128 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 2 & 5 & 0.012 & 41 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 2 & 111 & 0.146 & 98 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 2 & 5 & 0.021 & 90 \\ 
\end{tabular}
\begin{tabular}{|c|c|c|c|c|c|c|c|}\\  Source & Target & Num. vars & Related side & Arity & Variable & Before fix & After fix (%
  CMA 0 &  CMA 10 & 80 & True & 2 & 111 & 0.507 & 86 \\ 
 CMA 0 &  CMA 10 & 80 & True & 2 & 5 & 0.095 & 24 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 111 & 0.622 & 84 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 5 & 0.132 & 28 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 111 & 0.729 & 82 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 5 & 0.174 & 32 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 111 & 0.09 & 97 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 5 & 0.012 & 16 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 111 & 0.146 & 88 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 5 & 0.021 & 42 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 111 & 0.232 & 93 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 5 & 0.029 & 41 \\ 
 origin &  CMA 10 & 80 & True & 2 & 5 & 0.231 & 29 \\ 
 origin &  CMA 20 & 80 & True & 2 & 5 & 0.273 & 33 \\ 
 origin &  CMA 40 & 80 & True & 2 & 5 & 0.321 & 40 \\ 
 origin &  D1+1 10 & 80 & True & 2 & 5 & 0.142 & 30 \\ 
 origin &  D1+1 20 & 80 & True & 2 & 5 & 0.152 & 32 \\ 
 origin &  D1+1 40 & 80 & True & 2 & 5 & 0.16 & 26 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 111 & 0.507 & 99 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 5 & 0.095 & 92 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 111 & 0.622 & 100 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 5 & 0.132 & 97 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 111 & 0.729 & 99 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 5 & 0.174 & 100 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 2 & 111 & 0.09 & 128 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 2 & 5 & 0.012 & 41 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 2 & 111 & 0.146 & 98 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 2 & 5 & 0.021 & 90 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 2 & 111 & 0.232 & 98 \\ 
\end{tabular}
\begin{tabular}{|c|c|c|c|c|c|c|c|}\\  Source & Target & Num. vars & Related side & Arity & Variable & Before fix & After fix (%
  CMA 0 &  CMA 10 & 80 & True & 2 & 111 & 0.507 & 86 \\ 
 CMA 0 &  CMA 10 & 80 & True & 2 & 5 & 0.095 & 24 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 111 & 0.622 & 84 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 5 & 0.132 & 28 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 111 & 0.729 & 82 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 5 & 0.174 & 32 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 111 & 0.09 & 97 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 5 & 0.012 & 16 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 111 & 0.146 & 88 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 5 & 0.021 & 42 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 111 & 0.232 & 93 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 5 & 0.029 & 41 \\ 
 origin &  CMA 10 & 80 & True & 2 & 5 & 0.231 & 29 \\ 
 origin &  CMA 20 & 80 & True & 2 & 5 & 0.273 & 33 \\ 
 origin &  CMA 40 & 80 & True & 2 & 5 & 0.321 & 40 \\ 
 origin &  D1+1 10 & 80 & True & 2 & 5 & 0.142 & 30 \\ 
 origin &  D1+1 20 & 80 & True & 2 & 5 & 0.152 & 32 \\ 
 origin &  D1+1 40 & 80 & True & 2 & 5 & 0.16 & 26 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 111 & 0.507 & 99 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 5 & 0.095 & 92 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 111 & 0.622 & 100 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 5 & 0.132 & 97 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 111 & 0.729 & 99 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 5 & 0.174 & 100 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 2 & 111 & 0.09 & 128 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 2 & 5 & 0.012 & 41 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 2 & 111 & 0.146 & 98 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 2 & 5 & 0.021 & 90 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 2 & 111 & 0.232 & 98 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 2 & 5 & 0.029 & 17 \\ 
\end{tabular}
\begin{tabular}{|c|c|c|c|c|c|c|c|}\\  Source & Target & Num. vars & Related side & Arity & Variable & Before fix & After fix (%
  CMA 0 &  CMA 10 & 80 & True & 2 & 111 & 0.507 & 86 \\ 
 CMA 0 &  CMA 10 & 80 & True & 2 & 5 & 0.095 & 24 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 111 & 0.622 & 84 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 5 & 0.132 & 28 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 111 & 0.729 & 82 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 5 & 0.174 & 32 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 111 & 0.09 & 97 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 5 & 0.012 & 16 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 111 & 0.146 & 88 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 5 & 0.021 & 42 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 111 & 0.232 & 93 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 5 & 0.029 & 41 \\ 
 origin &  CMA 10 & 80 & True & 2 & 5 & 0.231 & 29 \\ 
 origin &  CMA 20 & 80 & True & 2 & 5 & 0.273 & 33 \\ 
 origin &  CMA 40 & 80 & True & 2 & 5 & 0.321 & 40 \\ 
 origin &  D1+1 10 & 80 & True & 2 & 5 & 0.142 & 30 \\ 
 origin &  D1+1 20 & 80 & True & 2 & 5 & 0.152 & 32 \\ 
 origin &  D1+1 40 & 80 & True & 2 & 5 & 0.16 & 26 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 111 & 0.507 & 99 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 5 & 0.095 & 92 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 111 & 0.622 & 100 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 5 & 0.132 & 97 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 111 & 0.729 & 99 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 5 & 0.174 & 100 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 2 & 111 & 0.09 & 128 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 2 & 5 & 0.012 & 41 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 2 & 111 & 0.146 & 98 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 2 & 5 & 0.021 & 90 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 2 & 111 & 0.232 & 98 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 2 & 5 & 0.029 & 17 \\ 
 origin &  CMA 10 & 1 & True & 2 & 5 & 0.231 & 53 \\ 
\end{tabular}
\begin{tabular}{|c|c|c|c|c|c|c|c|}\\  Source & Target & Num. vars & Related side & Arity & Variable & Before fix & After fix (%
  CMA 0 &  CMA 10 & 80 & True & 2 & 111 & 0.507 & 86 \\ 
 CMA 0 &  CMA 10 & 80 & True & 2 & 5 & 0.095 & 24 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 111 & 0.622 & 84 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 5 & 0.132 & 28 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 111 & 0.729 & 82 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 5 & 0.174 & 32 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 111 & 0.09 & 97 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 5 & 0.012 & 16 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 111 & 0.146 & 88 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 5 & 0.021 & 42 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 111 & 0.232 & 93 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 5 & 0.029 & 41 \\ 
 origin &  CMA 10 & 80 & True & 2 & 5 & 0.231 & 29 \\ 
 origin &  CMA 20 & 80 & True & 2 & 5 & 0.273 & 33 \\ 
 origin &  CMA 40 & 80 & True & 2 & 5 & 0.321 & 40 \\ 
 origin &  D1+1 10 & 80 & True & 2 & 5 & 0.142 & 30 \\ 
 origin &  D1+1 20 & 80 & True & 2 & 5 & 0.152 & 32 \\ 
 origin &  D1+1 40 & 80 & True & 2 & 5 & 0.16 & 26 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 111 & 0.507 & 99 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 5 & 0.095 & 92 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 111 & 0.622 & 100 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 5 & 0.132 & 97 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 111 & 0.729 & 99 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 5 & 0.174 & 100 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 2 & 111 & 0.09 & 128 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 2 & 5 & 0.012 & 41 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 2 & 111 & 0.146 & 98 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 2 & 5 & 0.021 & 90 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 2 & 111 & 0.232 & 98 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 2 & 5 & 0.029 & 17 \\ 
 origin &  CMA 10 & 1 & True & 2 & 5 & 0.231 & 53 \\ 
 origin &  CMA 20 & 1 & True & 2 & 5 & 0.273 & 53 \\ 
\end{tabular}
\begin{tabular}{|c|c|c|c|c|c|c|c|}\\  Source & Target & Num. vars & Related side & Arity & Variable & Before fix & After fix (%
  CMA 0 &  CMA 10 & 80 & True & 2 & 111 & 0.507 & 86 \\ 
 CMA 0 &  CMA 10 & 80 & True & 2 & 5 & 0.095 & 24 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 111 & 0.622 & 84 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 5 & 0.132 & 28 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 111 & 0.729 & 82 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 5 & 0.174 & 32 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 111 & 0.09 & 97 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 5 & 0.012 & 16 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 111 & 0.146 & 88 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 5 & 0.021 & 42 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 111 & 0.232 & 93 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 5 & 0.029 & 41 \\ 
 origin &  CMA 10 & 80 & True & 2 & 5 & 0.231 & 29 \\ 
 origin &  CMA 20 & 80 & True & 2 & 5 & 0.273 & 33 \\ 
 origin &  CMA 40 & 80 & True & 2 & 5 & 0.321 & 40 \\ 
 origin &  D1+1 10 & 80 & True & 2 & 5 & 0.142 & 30 \\ 
 origin &  D1+1 20 & 80 & True & 2 & 5 & 0.152 & 32 \\ 
 origin &  D1+1 40 & 80 & True & 2 & 5 & 0.16 & 26 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 111 & 0.507 & 99 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 5 & 0.095 & 92 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 111 & 0.622 & 100 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 5 & 0.132 & 97 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 111 & 0.729 & 99 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 5 & 0.174 & 100 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 2 & 111 & 0.09 & 128 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 2 & 5 & 0.012 & 41 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 2 & 111 & 0.146 & 98 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 2 & 5 & 0.021 & 90 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 2 & 111 & 0.232 & 98 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 2 & 5 & 0.029 & 17 \\ 
 origin &  CMA 10 & 1 & True & 2 & 5 & 0.231 & 53 \\ 
 origin &  CMA 20 & 1 & True & 2 & 5 & 0.273 & 53 \\ 
 origin &  CMA 40 & 1 & True & 2 & 5 & 0.321 & 67 \\ 
\end{tabular}
\begin{tabular}{|c|c|c|c|c|c|c|c|}\\  Source & Target & Num. vars & Related side & Arity & Variable & Before fix & After fix (%
  CMA 0 &  CMA 10 & 80 & True & 2 & 111 & 0.507 & 86 \\ 
 CMA 0 &  CMA 10 & 80 & True & 2 & 5 & 0.095 & 24 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 111 & 0.622 & 84 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 5 & 0.132 & 28 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 111 & 0.729 & 82 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 5 & 0.174 & 32 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 111 & 0.09 & 97 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 5 & 0.012 & 16 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 111 & 0.146 & 88 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 5 & 0.021 & 42 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 111 & 0.232 & 93 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 5 & 0.029 & 41 \\ 
 origin &  CMA 10 & 80 & True & 2 & 5 & 0.231 & 29 \\ 
 origin &  CMA 20 & 80 & True & 2 & 5 & 0.273 & 33 \\ 
 origin &  CMA 40 & 80 & True & 2 & 5 & 0.321 & 40 \\ 
 origin &  D1+1 10 & 80 & True & 2 & 5 & 0.142 & 30 \\ 
 origin &  D1+1 20 & 80 & True & 2 & 5 & 0.152 & 32 \\ 
 origin &  D1+1 40 & 80 & True & 2 & 5 & 0.16 & 26 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 111 & 0.507 & 99 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 5 & 0.095 & 92 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 111 & 0.622 & 100 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 5 & 0.132 & 97 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 111 & 0.729 & 99 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 5 & 0.174 & 100 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 2 & 111 & 0.09 & 128 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 2 & 5 & 0.012 & 41 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 2 & 111 & 0.146 & 98 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 2 & 5 & 0.021 & 90 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 2 & 111 & 0.232 & 98 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 2 & 5 & 0.029 & 17 \\ 
 origin &  CMA 10 & 1 & True & 2 & 5 & 0.231 & 53 \\ 
 origin &  CMA 20 & 1 & True & 2 & 5 & 0.273 & 53 \\ 
 origin &  CMA 40 & 1 & True & 2 & 5 & 0.321 & 67 \\ 
 origin &  D1+1 10 & 1 & True & 2 & 5 & 0.142 & 80 \\ 
\end{tabular}
\begin{tabular}{|c|c|c|c|c|c|c|c|}\\  Source & Target & Num. vars & Related side & Arity & Variable & Before fix & After fix (%
  CMA 0 &  CMA 10 & 80 & True & 2 & 111 & 0.507 & 86 \\ 
 CMA 0 &  CMA 10 & 80 & True & 2 & 5 & 0.095 & 24 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 111 & 0.622 & 84 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 5 & 0.132 & 28 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 111 & 0.729 & 82 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 5 & 0.174 & 32 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 111 & 0.09 & 97 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 5 & 0.012 & 16 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 111 & 0.146 & 88 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 5 & 0.021 & 42 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 111 & 0.232 & 93 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 5 & 0.029 & 41 \\ 
 origin &  CMA 10 & 80 & True & 2 & 5 & 0.231 & 29 \\ 
 origin &  CMA 20 & 80 & True & 2 & 5 & 0.273 & 33 \\ 
 origin &  CMA 40 & 80 & True & 2 & 5 & 0.321 & 40 \\ 
 origin &  D1+1 10 & 80 & True & 2 & 5 & 0.142 & 30 \\ 
 origin &  D1+1 20 & 80 & True & 2 & 5 & 0.152 & 32 \\ 
 origin &  D1+1 40 & 80 & True & 2 & 5 & 0.16 & 26 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 111 & 0.507 & 99 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 5 & 0.095 & 92 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 111 & 0.622 & 100 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 5 & 0.132 & 97 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 111 & 0.729 & 99 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 5 & 0.174 & 100 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 2 & 111 & 0.09 & 128 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 2 & 5 & 0.012 & 41 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 2 & 111 & 0.146 & 98 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 2 & 5 & 0.021 & 90 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 2 & 111 & 0.232 & 98 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 2 & 5 & 0.029 & 17 \\ 
 origin &  CMA 10 & 1 & True & 2 & 5 & 0.231 & 53 \\ 
 origin &  CMA 20 & 1 & True & 2 & 5 & 0.273 & 53 \\ 
 origin &  CMA 40 & 1 & True & 2 & 5 & 0.321 & 67 \\ 
 origin &  D1+1 10 & 1 & True & 2 & 5 & 0.142 & 80 \\ 
 origin &  D1+1 20 & 1 & True & 2 & 5 & 0.152 & 80 \\ 
\end{tabular}
\begin{tabular}{|c|c|c|c|c|c|c|c|}\\  Source & Target & Num. vars & Related side & Arity & Variable & Before fix & After fix (%
  CMA 0 &  CMA 10 & 80 & True & 2 & 111 & 0.507 & 86 \\ 
 CMA 0 &  CMA 10 & 80 & True & 2 & 5 & 0.095 & 24 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 111 & 0.622 & 84 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 5 & 0.132 & 28 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 111 & 0.729 & 82 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 5 & 0.174 & 32 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 111 & 0.09 & 97 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 5 & 0.012 & 16 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 111 & 0.146 & 88 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 5 & 0.021 & 42 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 111 & 0.232 & 93 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 5 & 0.029 & 41 \\ 
 origin &  CMA 10 & 80 & True & 2 & 5 & 0.231 & 29 \\ 
 origin &  CMA 20 & 80 & True & 2 & 5 & 0.273 & 33 \\ 
 origin &  CMA 40 & 80 & True & 2 & 5 & 0.321 & 40 \\ 
 origin &  D1+1 10 & 80 & True & 2 & 5 & 0.142 & 30 \\ 
 origin &  D1+1 20 & 80 & True & 2 & 5 & 0.152 & 32 \\ 
 origin &  D1+1 40 & 80 & True & 2 & 5 & 0.16 & 26 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 111 & 0.507 & 99 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 5 & 0.095 & 92 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 111 & 0.622 & 100 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 5 & 0.132 & 97 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 111 & 0.729 & 99 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 5 & 0.174 & 100 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 2 & 111 & 0.09 & 128 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 2 & 5 & 0.012 & 41 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 2 & 111 & 0.146 & 98 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 2 & 5 & 0.021 & 90 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 2 & 111 & 0.232 & 98 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 2 & 5 & 0.029 & 17 \\ 
 origin &  CMA 10 & 1 & True & 2 & 5 & 0.231 & 53 \\ 
 origin &  CMA 20 & 1 & True & 2 & 5 & 0.273 & 53 \\ 
 origin &  CMA 40 & 1 & True & 2 & 5 & 0.321 & 67 \\ 
 origin &  D1+1 10 & 1 & True & 2 & 5 & 0.142 & 80 \\ 
 origin &  D1+1 20 & 1 & True & 2 & 5 & 0.152 & 80 \\ 
 origin &  D1+1 40 & 1 & True & 2 & 5 & 0.16 & 80 \\ 
\end{tabular}
\begin{tabular}{|c|c|c|c|c|c|c|c|}\\  Source & Target & Num. vars & Related side & Arity & Variable & Before fix & After fix (%
  CMA 0 &  CMA 10 & 80 & True & 2 & 111 & 0.507 & 86 \\ 
 CMA 0 &  CMA 10 & 80 & True & 2 & 5 & 0.095 & 24 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 111 & 0.622 & 84 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 5 & 0.132 & 28 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 111 & 0.729 & 82 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 5 & 0.174 & 32 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 111 & 0.09 & 97 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 5 & 0.012 & 16 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 111 & 0.146 & 88 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 5 & 0.021 & 42 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 111 & 0.232 & 93 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 5 & 0.029 & 41 \\ 
 origin &  CMA 10 & 80 & True & 2 & 5 & 0.231 & 29 \\ 
 origin &  CMA 20 & 80 & True & 2 & 5 & 0.273 & 33 \\ 
 origin &  CMA 40 & 80 & True & 2 & 5 & 0.321 & 40 \\ 
 origin &  D1+1 10 & 80 & True & 2 & 5 & 0.142 & 30 \\ 
 origin &  D1+1 20 & 80 & True & 2 & 5 & 0.152 & 32 \\ 
 origin &  D1+1 40 & 80 & True & 2 & 5 & 0.16 & 26 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 111 & 0.507 & 99 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 5 & 0.095 & 92 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 111 & 0.622 & 100 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 5 & 0.132 & 97 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 111 & 0.729 & 99 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 5 & 0.174 & 100 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 2 & 111 & 0.09 & 128 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 2 & 5 & 0.012 & 41 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 2 & 111 & 0.146 & 98 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 2 & 5 & 0.021 & 90 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 2 & 111 & 0.232 & 98 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 2 & 5 & 0.029 & 17 \\ 
 origin &  CMA 10 & 1 & True & 2 & 5 & 0.231 & 53 \\ 
 origin &  CMA 20 & 1 & True & 2 & 5 & 0.273 & 53 \\ 
 origin &  CMA 40 & 1 & True & 2 & 5 & 0.321 & 67 \\ 
 origin &  D1+1 10 & 1 & True & 2 & 5 & 0.142 & 80 \\ 
 origin &  D1+1 20 & 1 & True & 2 & 5 & 0.152 & 80 \\ 
 origin &  D1+1 40 & 1 & True & 2 & 5 & 0.16 & 80 \\ 
 CMA 0 &  CMA 10 & 1 & True & 3 & 111 & 0.507 & 101 \\ 
\end{tabular}
\begin{tabular}{|c|c|c|c|c|c|c|c|}\\  Source & Target & Num. vars & Related side & Arity & Variable & Before fix & After fix (%
  CMA 0 &  CMA 10 & 80 & True & 2 & 111 & 0.507 & 86 \\ 
 CMA 0 &  CMA 10 & 80 & True & 2 & 5 & 0.095 & 24 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 111 & 0.622 & 84 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 5 & 0.132 & 28 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 111 & 0.729 & 82 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 5 & 0.174 & 32 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 111 & 0.09 & 97 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 5 & 0.012 & 16 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 111 & 0.146 & 88 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 5 & 0.021 & 42 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 111 & 0.232 & 93 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 5 & 0.029 & 41 \\ 
 origin &  CMA 10 & 80 & True & 2 & 5 & 0.231 & 29 \\ 
 origin &  CMA 20 & 80 & True & 2 & 5 & 0.273 & 33 \\ 
 origin &  CMA 40 & 80 & True & 2 & 5 & 0.321 & 40 \\ 
 origin &  D1+1 10 & 80 & True & 2 & 5 & 0.142 & 30 \\ 
 origin &  D1+1 20 & 80 & True & 2 & 5 & 0.152 & 32 \\ 
 origin &  D1+1 40 & 80 & True & 2 & 5 & 0.16 & 26 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 111 & 0.507 & 99 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 5 & 0.095 & 92 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 111 & 0.622 & 100 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 5 & 0.132 & 97 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 111 & 0.729 & 99 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 5 & 0.174 & 100 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 2 & 111 & 0.09 & 128 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 2 & 5 & 0.012 & 41 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 2 & 111 & 0.146 & 98 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 2 & 5 & 0.021 & 90 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 2 & 111 & 0.232 & 98 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 2 & 5 & 0.029 & 17 \\ 
 origin &  CMA 10 & 1 & True & 2 & 5 & 0.231 & 53 \\ 
 origin &  CMA 20 & 1 & True & 2 & 5 & 0.273 & 53 \\ 
 origin &  CMA 40 & 1 & True & 2 & 5 & 0.321 & 67 \\ 
 origin &  D1+1 10 & 1 & True & 2 & 5 & 0.142 & 80 \\ 
 origin &  D1+1 20 & 1 & True & 2 & 5 & 0.152 & 80 \\ 
 origin &  D1+1 40 & 1 & True & 2 & 5 & 0.16 & 80 \\ 
 CMA 0 &  CMA 10 & 1 & True & 3 & 111 & 0.507 & 101 \\ 
 CMA 0 &  CMA 10 & 1 & True & 3 & 5 & 0.095 & 97 \\ 
\end{tabular}
\begin{tabular}{|c|c|c|c|c|c|c|c|}\\  Source & Target & Num. vars & Related side & Arity & Variable & Before fix & After fix (%
  CMA 0 &  CMA 10 & 80 & True & 2 & 111 & 0.507 & 86 \\ 
 CMA 0 &  CMA 10 & 80 & True & 2 & 5 & 0.095 & 24 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 111 & 0.622 & 84 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 5 & 0.132 & 28 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 111 & 0.729 & 82 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 5 & 0.174 & 32 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 111 & 0.09 & 97 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 5 & 0.012 & 16 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 111 & 0.146 & 88 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 5 & 0.021 & 42 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 111 & 0.232 & 93 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 5 & 0.029 & 41 \\ 
 origin &  CMA 10 & 80 & True & 2 & 5 & 0.231 & 29 \\ 
 origin &  CMA 20 & 80 & True & 2 & 5 & 0.273 & 33 \\ 
 origin &  CMA 40 & 80 & True & 2 & 5 & 0.321 & 40 \\ 
 origin &  D1+1 10 & 80 & True & 2 & 5 & 0.142 & 30 \\ 
 origin &  D1+1 20 & 80 & True & 2 & 5 & 0.152 & 32 \\ 
 origin &  D1+1 40 & 80 & True & 2 & 5 & 0.16 & 26 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 111 & 0.507 & 99 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 5 & 0.095 & 92 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 111 & 0.622 & 100 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 5 & 0.132 & 97 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 111 & 0.729 & 99 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 5 & 0.174 & 100 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 2 & 111 & 0.09 & 128 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 2 & 5 & 0.012 & 41 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 2 & 111 & 0.146 & 98 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 2 & 5 & 0.021 & 90 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 2 & 111 & 0.232 & 98 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 2 & 5 & 0.029 & 17 \\ 
 origin &  CMA 10 & 1 & True & 2 & 5 & 0.231 & 53 \\ 
 origin &  CMA 20 & 1 & True & 2 & 5 & 0.273 & 53 \\ 
 origin &  CMA 40 & 1 & True & 2 & 5 & 0.321 & 67 \\ 
 origin &  D1+1 10 & 1 & True & 2 & 5 & 0.142 & 80 \\ 
 origin &  D1+1 20 & 1 & True & 2 & 5 & 0.152 & 80 \\ 
 origin &  D1+1 40 & 1 & True & 2 & 5 & 0.16 & 80 \\ 
 CMA 0 &  CMA 10 & 1 & True & 3 & 111 & 0.507 & 101 \\ 
 CMA 0 &  CMA 10 & 1 & True & 3 & 5 & 0.095 & 97 \\ 
 CMA 0 &  CMA 20 & 1 & True & 3 & 111 & 0.622 & 100 \\ 
\end{tabular}
\begin{tabular}{|c|c|c|c|c|c|c|c|}\\  Source & Target & Num. vars & Related side & Arity & Variable & Before fix & After fix (%
  CMA 0 &  CMA 10 & 80 & True & 2 & 111 & 0.507 & 86 \\ 
 CMA 0 &  CMA 10 & 80 & True & 2 & 5 & 0.095 & 24 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 111 & 0.622 & 84 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 5 & 0.132 & 28 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 111 & 0.729 & 82 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 5 & 0.174 & 32 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 111 & 0.09 & 97 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 5 & 0.012 & 16 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 111 & 0.146 & 88 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 5 & 0.021 & 42 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 111 & 0.232 & 93 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 5 & 0.029 & 41 \\ 
 origin &  CMA 10 & 80 & True & 2 & 5 & 0.231 & 29 \\ 
 origin &  CMA 20 & 80 & True & 2 & 5 & 0.273 & 33 \\ 
 origin &  CMA 40 & 80 & True & 2 & 5 & 0.321 & 40 \\ 
 origin &  D1+1 10 & 80 & True & 2 & 5 & 0.142 & 30 \\ 
 origin &  D1+1 20 & 80 & True & 2 & 5 & 0.152 & 32 \\ 
 origin &  D1+1 40 & 80 & True & 2 & 5 & 0.16 & 26 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 111 & 0.507 & 99 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 5 & 0.095 & 92 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 111 & 0.622 & 100 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 5 & 0.132 & 97 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 111 & 0.729 & 99 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 5 & 0.174 & 100 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 2 & 111 & 0.09 & 128 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 2 & 5 & 0.012 & 41 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 2 & 111 & 0.146 & 98 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 2 & 5 & 0.021 & 90 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 2 & 111 & 0.232 & 98 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 2 & 5 & 0.029 & 17 \\ 
 origin &  CMA 10 & 1 & True & 2 & 5 & 0.231 & 53 \\ 
 origin &  CMA 20 & 1 & True & 2 & 5 & 0.273 & 53 \\ 
 origin &  CMA 40 & 1 & True & 2 & 5 & 0.321 & 67 \\ 
 origin &  D1+1 10 & 1 & True & 2 & 5 & 0.142 & 80 \\ 
 origin &  D1+1 20 & 1 & True & 2 & 5 & 0.152 & 80 \\ 
 origin &  D1+1 40 & 1 & True & 2 & 5 & 0.16 & 80 \\ 
 CMA 0 &  CMA 10 & 1 & True & 3 & 111 & 0.507 & 101 \\ 
 CMA 0 &  CMA 10 & 1 & True & 3 & 5 & 0.095 & 97 \\ 
 CMA 0 &  CMA 20 & 1 & True & 3 & 111 & 0.622 & 100 \\ 
 CMA 0 &  CMA 20 & 1 & True & 3 & 5 & 0.132 & 97 \\ 
\end{tabular}
\begin{tabular}{|c|c|c|c|c|c|c|c|}\\  Source & Target & Num. vars & Related side & Arity & Variable & Before fix & After fix (%
  CMA 0 &  CMA 10 & 80 & True & 2 & 111 & 0.507 & 86 \\ 
 CMA 0 &  CMA 10 & 80 & True & 2 & 5 & 0.095 & 24 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 111 & 0.622 & 84 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 5 & 0.132 & 28 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 111 & 0.729 & 82 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 5 & 0.174 & 32 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 111 & 0.09 & 97 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 5 & 0.012 & 16 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 111 & 0.146 & 88 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 5 & 0.021 & 42 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 111 & 0.232 & 93 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 5 & 0.029 & 41 \\ 
 origin &  CMA 10 & 80 & True & 2 & 5 & 0.231 & 29 \\ 
 origin &  CMA 20 & 80 & True & 2 & 5 & 0.273 & 33 \\ 
 origin &  CMA 40 & 80 & True & 2 & 5 & 0.321 & 40 \\ 
 origin &  D1+1 10 & 80 & True & 2 & 5 & 0.142 & 30 \\ 
 origin &  D1+1 20 & 80 & True & 2 & 5 & 0.152 & 32 \\ 
 origin &  D1+1 40 & 80 & True & 2 & 5 & 0.16 & 26 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 111 & 0.507 & 99 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 5 & 0.095 & 92 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 111 & 0.622 & 100 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 5 & 0.132 & 97 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 111 & 0.729 & 99 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 5 & 0.174 & 100 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 2 & 111 & 0.09 & 128 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 2 & 5 & 0.012 & 41 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 2 & 111 & 0.146 & 98 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 2 & 5 & 0.021 & 90 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 2 & 111 & 0.232 & 98 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 2 & 5 & 0.029 & 17 \\ 
 origin &  CMA 10 & 1 & True & 2 & 5 & 0.231 & 53 \\ 
 origin &  CMA 20 & 1 & True & 2 & 5 & 0.273 & 53 \\ 
 origin &  CMA 40 & 1 & True & 2 & 5 & 0.321 & 67 \\ 
 origin &  D1+1 10 & 1 & True & 2 & 5 & 0.142 & 80 \\ 
 origin &  D1+1 20 & 1 & True & 2 & 5 & 0.152 & 80 \\ 
 origin &  D1+1 40 & 1 & True & 2 & 5 & 0.16 & 80 \\ 
 CMA 0 &  CMA 10 & 1 & True & 3 & 111 & 0.507 & 101 \\ 
 CMA 0 &  CMA 10 & 1 & True & 3 & 5 & 0.095 & 97 \\ 
 CMA 0 &  CMA 20 & 1 & True & 3 & 111 & 0.622 & 100 \\ 
 CMA 0 &  CMA 20 & 1 & True & 3 & 5 & 0.132 & 97 \\ 
 CMA 0 &  CMA 40 & 1 & True & 3 & 111 & 0.729 & 98 \\ 
\end{tabular}
\begin{tabular}{|c|c|c|c|c|c|c|c|}\\  Source & Target & Num. vars & Related side & Arity & Variable & Before fix & After fix (%
  CMA 0 &  CMA 10 & 80 & True & 2 & 111 & 0.507 & 86 \\ 
 CMA 0 &  CMA 10 & 80 & True & 2 & 5 & 0.095 & 24 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 111 & 0.622 & 84 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 5 & 0.132 & 28 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 111 & 0.729 & 82 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 5 & 0.174 & 32 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 111 & 0.09 & 97 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 5 & 0.012 & 16 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 111 & 0.146 & 88 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 5 & 0.021 & 42 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 111 & 0.232 & 93 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 5 & 0.029 & 41 \\ 
 origin &  CMA 10 & 80 & True & 2 & 5 & 0.231 & 29 \\ 
 origin &  CMA 20 & 80 & True & 2 & 5 & 0.273 & 33 \\ 
 origin &  CMA 40 & 80 & True & 2 & 5 & 0.321 & 40 \\ 
 origin &  D1+1 10 & 80 & True & 2 & 5 & 0.142 & 30 \\ 
 origin &  D1+1 20 & 80 & True & 2 & 5 & 0.152 & 32 \\ 
 origin &  D1+1 40 & 80 & True & 2 & 5 & 0.16 & 26 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 111 & 0.507 & 99 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 5 & 0.095 & 92 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 111 & 0.622 & 100 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 5 & 0.132 & 97 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 111 & 0.729 & 99 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 5 & 0.174 & 100 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 2 & 111 & 0.09 & 128 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 2 & 5 & 0.012 & 41 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 2 & 111 & 0.146 & 98 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 2 & 5 & 0.021 & 90 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 2 & 111 & 0.232 & 98 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 2 & 5 & 0.029 & 17 \\ 
 origin &  CMA 10 & 1 & True & 2 & 5 & 0.231 & 53 \\ 
 origin &  CMA 20 & 1 & True & 2 & 5 & 0.273 & 53 \\ 
 origin &  CMA 40 & 1 & True & 2 & 5 & 0.321 & 67 \\ 
 origin &  D1+1 10 & 1 & True & 2 & 5 & 0.142 & 80 \\ 
 origin &  D1+1 20 & 1 & True & 2 & 5 & 0.152 & 80 \\ 
 origin &  D1+1 40 & 1 & True & 2 & 5 & 0.16 & 80 \\ 
 CMA 0 &  CMA 10 & 1 & True & 3 & 111 & 0.507 & 101 \\ 
 CMA 0 &  CMA 10 & 1 & True & 3 & 5 & 0.095 & 97 \\ 
 CMA 0 &  CMA 20 & 1 & True & 3 & 111 & 0.622 & 100 \\ 
 CMA 0 &  CMA 20 & 1 & True & 3 & 5 & 0.132 & 97 \\ 
 CMA 0 &  CMA 40 & 1 & True & 3 & 111 & 0.729 & 98 \\ 
 CMA 0 &  CMA 40 & 1 & True & 3 & 5 & 0.174 & 88 \\ 
\end{tabular}
\begin{tabular}{|c|c|c|c|c|c|c|c|}\\  Source & Target & Num. vars & Related side & Arity & Variable & Before fix & After fix (%
  CMA 0 &  CMA 10 & 80 & True & 2 & 111 & 0.507 & 86 \\ 
 CMA 0 &  CMA 10 & 80 & True & 2 & 5 & 0.095 & 24 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 111 & 0.622 & 84 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 5 & 0.132 & 28 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 111 & 0.729 & 82 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 5 & 0.174 & 32 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 111 & 0.09 & 97 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 5 & 0.012 & 16 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 111 & 0.146 & 88 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 5 & 0.021 & 42 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 111 & 0.232 & 93 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 5 & 0.029 & 41 \\ 
 origin &  CMA 10 & 80 & True & 2 & 5 & 0.231 & 29 \\ 
 origin &  CMA 20 & 80 & True & 2 & 5 & 0.273 & 33 \\ 
 origin &  CMA 40 & 80 & True & 2 & 5 & 0.321 & 40 \\ 
 origin &  D1+1 10 & 80 & True & 2 & 5 & 0.142 & 30 \\ 
 origin &  D1+1 20 & 80 & True & 2 & 5 & 0.152 & 32 \\ 
 origin &  D1+1 40 & 80 & True & 2 & 5 & 0.16 & 26 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 111 & 0.507 & 99 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 5 & 0.095 & 92 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 111 & 0.622 & 100 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 5 & 0.132 & 97 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 111 & 0.729 & 99 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 5 & 0.174 & 100 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 2 & 111 & 0.09 & 128 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 2 & 5 & 0.012 & 41 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 2 & 111 & 0.146 & 98 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 2 & 5 & 0.021 & 90 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 2 & 111 & 0.232 & 98 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 2 & 5 & 0.029 & 17 \\ 
 origin &  CMA 10 & 1 & True & 2 & 5 & 0.231 & 53 \\ 
 origin &  CMA 20 & 1 & True & 2 & 5 & 0.273 & 53 \\ 
 origin &  CMA 40 & 1 & True & 2 & 5 & 0.321 & 67 \\ 
 origin &  D1+1 10 & 1 & True & 2 & 5 & 0.142 & 80 \\ 
 origin &  D1+1 20 & 1 & True & 2 & 5 & 0.152 & 80 \\ 
 origin &  D1+1 40 & 1 & True & 2 & 5 & 0.16 & 80 \\ 
 CMA 0 &  CMA 10 & 1 & True & 3 & 111 & 0.507 & 101 \\ 
 CMA 0 &  CMA 10 & 1 & True & 3 & 5 & 0.095 & 97 \\ 
 CMA 0 &  CMA 20 & 1 & True & 3 & 111 & 0.622 & 100 \\ 
 CMA 0 &  CMA 20 & 1 & True & 3 & 5 & 0.132 & 97 \\ 
 CMA 0 &  CMA 40 & 1 & True & 3 & 111 & 0.729 & 98 \\ 
 CMA 0 &  CMA 40 & 1 & True & 3 & 5 & 0.174 & 88 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 3 & 111 & 0.09 & 102 \\ 
\end{tabular}
\begin{tabular}{|c|c|c|c|c|c|c|c|}\\  Source & Target & Num. vars & Related side & Arity & Variable & Before fix & After fix (%
  CMA 0 &  CMA 10 & 80 & True & 2 & 111 & 0.507 & 86 \\ 
 CMA 0 &  CMA 10 & 80 & True & 2 & 5 & 0.095 & 24 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 111 & 0.622 & 84 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 5 & 0.132 & 28 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 111 & 0.729 & 82 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 5 & 0.174 & 32 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 111 & 0.09 & 97 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 5 & 0.012 & 16 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 111 & 0.146 & 88 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 5 & 0.021 & 42 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 111 & 0.232 & 93 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 5 & 0.029 & 41 \\ 
 origin &  CMA 10 & 80 & True & 2 & 5 & 0.231 & 29 \\ 
 origin &  CMA 20 & 80 & True & 2 & 5 & 0.273 & 33 \\ 
 origin &  CMA 40 & 80 & True & 2 & 5 & 0.321 & 40 \\ 
 origin &  D1+1 10 & 80 & True & 2 & 5 & 0.142 & 30 \\ 
 origin &  D1+1 20 & 80 & True & 2 & 5 & 0.152 & 32 \\ 
 origin &  D1+1 40 & 80 & True & 2 & 5 & 0.16 & 26 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 111 & 0.507 & 99 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 5 & 0.095 & 92 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 111 & 0.622 & 100 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 5 & 0.132 & 97 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 111 & 0.729 & 99 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 5 & 0.174 & 100 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 2 & 111 & 0.09 & 128 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 2 & 5 & 0.012 & 41 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 2 & 111 & 0.146 & 98 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 2 & 5 & 0.021 & 90 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 2 & 111 & 0.232 & 98 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 2 & 5 & 0.029 & 17 \\ 
 origin &  CMA 10 & 1 & True & 2 & 5 & 0.231 & 53 \\ 
 origin &  CMA 20 & 1 & True & 2 & 5 & 0.273 & 53 \\ 
 origin &  CMA 40 & 1 & True & 2 & 5 & 0.321 & 67 \\ 
 origin &  D1+1 10 & 1 & True & 2 & 5 & 0.142 & 80 \\ 
 origin &  D1+1 20 & 1 & True & 2 & 5 & 0.152 & 80 \\ 
 origin &  D1+1 40 & 1 & True & 2 & 5 & 0.16 & 80 \\ 
 CMA 0 &  CMA 10 & 1 & True & 3 & 111 & 0.507 & 101 \\ 
 CMA 0 &  CMA 10 & 1 & True & 3 & 5 & 0.095 & 97 \\ 
 CMA 0 &  CMA 20 & 1 & True & 3 & 111 & 0.622 & 100 \\ 
 CMA 0 &  CMA 20 & 1 & True & 3 & 5 & 0.132 & 97 \\ 
 CMA 0 &  CMA 40 & 1 & True & 3 & 111 & 0.729 & 98 \\ 
 CMA 0 &  CMA 40 & 1 & True & 3 & 5 & 0.174 & 88 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 3 & 111 & 0.09 & 102 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 3 & 5 & 0.012 & 83 \\ 
\end{tabular}
\begin{tabular}{|c|c|c|c|c|c|c|c|}\\  Source & Target & Num. vars & Related side & Arity & Variable & Before fix & After fix (%
  CMA 0 &  CMA 10 & 80 & True & 2 & 111 & 0.507 & 86 \\ 
 CMA 0 &  CMA 10 & 80 & True & 2 & 5 & 0.095 & 24 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 111 & 0.622 & 84 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 5 & 0.132 & 28 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 111 & 0.729 & 82 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 5 & 0.174 & 32 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 111 & 0.09 & 97 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 5 & 0.012 & 16 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 111 & 0.146 & 88 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 5 & 0.021 & 42 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 111 & 0.232 & 93 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 5 & 0.029 & 41 \\ 
 origin &  CMA 10 & 80 & True & 2 & 5 & 0.231 & 29 \\ 
 origin &  CMA 20 & 80 & True & 2 & 5 & 0.273 & 33 \\ 
 origin &  CMA 40 & 80 & True & 2 & 5 & 0.321 & 40 \\ 
 origin &  D1+1 10 & 80 & True & 2 & 5 & 0.142 & 30 \\ 
 origin &  D1+1 20 & 80 & True & 2 & 5 & 0.152 & 32 \\ 
 origin &  D1+1 40 & 80 & True & 2 & 5 & 0.16 & 26 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 111 & 0.507 & 99 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 5 & 0.095 & 92 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 111 & 0.622 & 100 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 5 & 0.132 & 97 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 111 & 0.729 & 99 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 5 & 0.174 & 100 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 2 & 111 & 0.09 & 128 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 2 & 5 & 0.012 & 41 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 2 & 111 & 0.146 & 98 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 2 & 5 & 0.021 & 90 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 2 & 111 & 0.232 & 98 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 2 & 5 & 0.029 & 17 \\ 
 origin &  CMA 10 & 1 & True & 2 & 5 & 0.231 & 53 \\ 
 origin &  CMA 20 & 1 & True & 2 & 5 & 0.273 & 53 \\ 
 origin &  CMA 40 & 1 & True & 2 & 5 & 0.321 & 67 \\ 
 origin &  D1+1 10 & 1 & True & 2 & 5 & 0.142 & 80 \\ 
 origin &  D1+1 20 & 1 & True & 2 & 5 & 0.152 & 80 \\ 
 origin &  D1+1 40 & 1 & True & 2 & 5 & 0.16 & 80 \\ 
 CMA 0 &  CMA 10 & 1 & True & 3 & 111 & 0.507 & 101 \\ 
 CMA 0 &  CMA 10 & 1 & True & 3 & 5 & 0.095 & 97 \\ 
 CMA 0 &  CMA 20 & 1 & True & 3 & 111 & 0.622 & 100 \\ 
 CMA 0 &  CMA 20 & 1 & True & 3 & 5 & 0.132 & 97 \\ 
 CMA 0 &  CMA 40 & 1 & True & 3 & 111 & 0.729 & 98 \\ 
 CMA 0 &  CMA 40 & 1 & True & 3 & 5 & 0.174 & 88 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 3 & 111 & 0.09 & 102 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 3 & 5 & 0.012 & 83 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 3 & 111 & 0.146 & 100 \\ 
\end{tabular}
\begin{tabular}{|c|c|c|c|c|c|c|c|}\\  Source & Target & Num. vars & Related side & Arity & Variable & Before fix & After fix (%
  CMA 0 &  CMA 10 & 80 & True & 2 & 111 & 0.507 & 86 \\ 
 CMA 0 &  CMA 10 & 80 & True & 2 & 5 & 0.095 & 24 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 111 & 0.622 & 84 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 5 & 0.132 & 28 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 111 & 0.729 & 82 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 5 & 0.174 & 32 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 111 & 0.09 & 97 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 5 & 0.012 & 16 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 111 & 0.146 & 88 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 5 & 0.021 & 42 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 111 & 0.232 & 93 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 5 & 0.029 & 41 \\ 
 origin &  CMA 10 & 80 & True & 2 & 5 & 0.231 & 29 \\ 
 origin &  CMA 20 & 80 & True & 2 & 5 & 0.273 & 33 \\ 
 origin &  CMA 40 & 80 & True & 2 & 5 & 0.321 & 40 \\ 
 origin &  D1+1 10 & 80 & True & 2 & 5 & 0.142 & 30 \\ 
 origin &  D1+1 20 & 80 & True & 2 & 5 & 0.152 & 32 \\ 
 origin &  D1+1 40 & 80 & True & 2 & 5 & 0.16 & 26 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 111 & 0.507 & 99 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 5 & 0.095 & 92 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 111 & 0.622 & 100 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 5 & 0.132 & 97 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 111 & 0.729 & 99 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 5 & 0.174 & 100 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 2 & 111 & 0.09 & 128 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 2 & 5 & 0.012 & 41 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 2 & 111 & 0.146 & 98 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 2 & 5 & 0.021 & 90 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 2 & 111 & 0.232 & 98 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 2 & 5 & 0.029 & 17 \\ 
 origin &  CMA 10 & 1 & True & 2 & 5 & 0.231 & 53 \\ 
 origin &  CMA 20 & 1 & True & 2 & 5 & 0.273 & 53 \\ 
 origin &  CMA 40 & 1 & True & 2 & 5 & 0.321 & 67 \\ 
 origin &  D1+1 10 & 1 & True & 2 & 5 & 0.142 & 80 \\ 
 origin &  D1+1 20 & 1 & True & 2 & 5 & 0.152 & 80 \\ 
 origin &  D1+1 40 & 1 & True & 2 & 5 & 0.16 & 80 \\ 
 CMA 0 &  CMA 10 & 1 & True & 3 & 111 & 0.507 & 101 \\ 
 CMA 0 &  CMA 10 & 1 & True & 3 & 5 & 0.095 & 97 \\ 
 CMA 0 &  CMA 20 & 1 & True & 3 & 111 & 0.622 & 100 \\ 
 CMA 0 &  CMA 20 & 1 & True & 3 & 5 & 0.132 & 97 \\ 
 CMA 0 &  CMA 40 & 1 & True & 3 & 111 & 0.729 & 98 \\ 
 CMA 0 &  CMA 40 & 1 & True & 3 & 5 & 0.174 & 88 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 3 & 111 & 0.09 & 102 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 3 & 5 & 0.012 & 83 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 3 & 111 & 0.146 & 100 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 3 & 5 & 0.021 & 38 \\ 
\end{tabular}
\begin{tabular}{|c|c|c|c|c|c|c|c|}\\  Source & Target & Num. vars & Related side & Arity & Variable & Before fix & After fix (%
  CMA 0 &  CMA 10 & 80 & True & 2 & 111 & 0.507 & 86 \\ 
 CMA 0 &  CMA 10 & 80 & True & 2 & 5 & 0.095 & 24 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 111 & 0.622 & 84 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 5 & 0.132 & 28 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 111 & 0.729 & 82 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 5 & 0.174 & 32 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 111 & 0.09 & 97 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 5 & 0.012 & 16 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 111 & 0.146 & 88 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 5 & 0.021 & 42 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 111 & 0.232 & 93 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 5 & 0.029 & 41 \\ 
 origin &  CMA 10 & 80 & True & 2 & 5 & 0.231 & 29 \\ 
 origin &  CMA 20 & 80 & True & 2 & 5 & 0.273 & 33 \\ 
 origin &  CMA 40 & 80 & True & 2 & 5 & 0.321 & 40 \\ 
 origin &  D1+1 10 & 80 & True & 2 & 5 & 0.142 & 30 \\ 
 origin &  D1+1 20 & 80 & True & 2 & 5 & 0.152 & 32 \\ 
 origin &  D1+1 40 & 80 & True & 2 & 5 & 0.16 & 26 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 111 & 0.507 & 99 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 5 & 0.095 & 92 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 111 & 0.622 & 100 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 5 & 0.132 & 97 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 111 & 0.729 & 99 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 5 & 0.174 & 100 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 2 & 111 & 0.09 & 128 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 2 & 5 & 0.012 & 41 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 2 & 111 & 0.146 & 98 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 2 & 5 & 0.021 & 90 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 2 & 111 & 0.232 & 98 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 2 & 5 & 0.029 & 17 \\ 
 origin &  CMA 10 & 1 & True & 2 & 5 & 0.231 & 53 \\ 
 origin &  CMA 20 & 1 & True & 2 & 5 & 0.273 & 53 \\ 
 origin &  CMA 40 & 1 & True & 2 & 5 & 0.321 & 67 \\ 
 origin &  D1+1 10 & 1 & True & 2 & 5 & 0.142 & 80 \\ 
 origin &  D1+1 20 & 1 & True & 2 & 5 & 0.152 & 80 \\ 
 origin &  D1+1 40 & 1 & True & 2 & 5 & 0.16 & 80 \\ 
 CMA 0 &  CMA 10 & 1 & True & 3 & 111 & 0.507 & 101 \\ 
 CMA 0 &  CMA 10 & 1 & True & 3 & 5 & 0.095 & 97 \\ 
 CMA 0 &  CMA 20 & 1 & True & 3 & 111 & 0.622 & 100 \\ 
 CMA 0 &  CMA 20 & 1 & True & 3 & 5 & 0.132 & 97 \\ 
 CMA 0 &  CMA 40 & 1 & True & 3 & 111 & 0.729 & 98 \\ 
 CMA 0 &  CMA 40 & 1 & True & 3 & 5 & 0.174 & 88 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 3 & 111 & 0.09 & 102 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 3 & 5 & 0.012 & 83 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 3 & 111 & 0.146 & 100 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 3 & 5 & 0.021 & 38 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 3 & 111 & 0.232 & 91 \\ 
\end{tabular}
\begin{tabular}{|c|c|c|c|c|c|c|c|}\\  Source & Target & Num. vars & Related side & Arity & Variable & Before fix & After fix (%
  CMA 0 &  CMA 10 & 80 & True & 2 & 111 & 0.507 & 86 \\ 
 CMA 0 &  CMA 10 & 80 & True & 2 & 5 & 0.095 & 24 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 111 & 0.622 & 84 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 5 & 0.132 & 28 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 111 & 0.729 & 82 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 5 & 0.174 & 32 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 111 & 0.09 & 97 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 5 & 0.012 & 16 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 111 & 0.146 & 88 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 5 & 0.021 & 42 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 111 & 0.232 & 93 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 5 & 0.029 & 41 \\ 
 origin &  CMA 10 & 80 & True & 2 & 5 & 0.231 & 29 \\ 
 origin &  CMA 20 & 80 & True & 2 & 5 & 0.273 & 33 \\ 
 origin &  CMA 40 & 80 & True & 2 & 5 & 0.321 & 40 \\ 
 origin &  D1+1 10 & 80 & True & 2 & 5 & 0.142 & 30 \\ 
 origin &  D1+1 20 & 80 & True & 2 & 5 & 0.152 & 32 \\ 
 origin &  D1+1 40 & 80 & True & 2 & 5 & 0.16 & 26 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 111 & 0.507 & 99 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 5 & 0.095 & 92 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 111 & 0.622 & 100 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 5 & 0.132 & 97 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 111 & 0.729 & 99 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 5 & 0.174 & 100 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 2 & 111 & 0.09 & 128 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 2 & 5 & 0.012 & 41 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 2 & 111 & 0.146 & 98 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 2 & 5 & 0.021 & 90 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 2 & 111 & 0.232 & 98 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 2 & 5 & 0.029 & 17 \\ 
 origin &  CMA 10 & 1 & True & 2 & 5 & 0.231 & 53 \\ 
 origin &  CMA 20 & 1 & True & 2 & 5 & 0.273 & 53 \\ 
 origin &  CMA 40 & 1 & True & 2 & 5 & 0.321 & 67 \\ 
 origin &  D1+1 10 & 1 & True & 2 & 5 & 0.142 & 80 \\ 
 origin &  D1+1 20 & 1 & True & 2 & 5 & 0.152 & 80 \\ 
 origin &  D1+1 40 & 1 & True & 2 & 5 & 0.16 & 80 \\ 
 CMA 0 &  CMA 10 & 1 & True & 3 & 111 & 0.507 & 101 \\ 
 CMA 0 &  CMA 10 & 1 & True & 3 & 5 & 0.095 & 97 \\ 
 CMA 0 &  CMA 20 & 1 & True & 3 & 111 & 0.622 & 100 \\ 
 CMA 0 &  CMA 20 & 1 & True & 3 & 5 & 0.132 & 97 \\ 
 CMA 0 &  CMA 40 & 1 & True & 3 & 111 & 0.729 & 98 \\ 
 CMA 0 &  CMA 40 & 1 & True & 3 & 5 & 0.174 & 88 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 3 & 111 & 0.09 & 102 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 3 & 5 & 0.012 & 83 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 3 & 111 & 0.146 & 100 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 3 & 5 & 0.021 & 38 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 3 & 111 & 0.232 & 91 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 3 & 5 & 0.029 & 41 \\ 
\end{tabular}
\begin{tabular}{|c|c|c|c|c|c|c|c|}\\  Source & Target & Num. vars & Related side & Arity & Variable & Before fix & After fix (%
  CMA 0 &  CMA 10 & 80 & True & 2 & 111 & 0.507 & 86 \\ 
 CMA 0 &  CMA 10 & 80 & True & 2 & 5 & 0.095 & 24 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 111 & 0.622 & 84 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 5 & 0.132 & 28 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 111 & 0.729 & 82 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 5 & 0.174 & 32 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 111 & 0.09 & 97 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 5 & 0.012 & 16 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 111 & 0.146 & 88 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 5 & 0.021 & 42 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 111 & 0.232 & 93 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 5 & 0.029 & 41 \\ 
 origin &  CMA 10 & 80 & True & 2 & 5 & 0.231 & 29 \\ 
 origin &  CMA 20 & 80 & True & 2 & 5 & 0.273 & 33 \\ 
 origin &  CMA 40 & 80 & True & 2 & 5 & 0.321 & 40 \\ 
 origin &  D1+1 10 & 80 & True & 2 & 5 & 0.142 & 30 \\ 
 origin &  D1+1 20 & 80 & True & 2 & 5 & 0.152 & 32 \\ 
 origin &  D1+1 40 & 80 & True & 2 & 5 & 0.16 & 26 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 111 & 0.507 & 99 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 5 & 0.095 & 92 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 111 & 0.622 & 100 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 5 & 0.132 & 97 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 111 & 0.729 & 99 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 5 & 0.174 & 100 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 2 & 111 & 0.09 & 128 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 2 & 5 & 0.012 & 41 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 2 & 111 & 0.146 & 98 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 2 & 5 & 0.021 & 90 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 2 & 111 & 0.232 & 98 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 2 & 5 & 0.029 & 17 \\ 
 origin &  CMA 10 & 1 & True & 2 & 5 & 0.231 & 53 \\ 
 origin &  CMA 20 & 1 & True & 2 & 5 & 0.273 & 53 \\ 
 origin &  CMA 40 & 1 & True & 2 & 5 & 0.321 & 67 \\ 
 origin &  D1+1 10 & 1 & True & 2 & 5 & 0.142 & 80 \\ 
 origin &  D1+1 20 & 1 & True & 2 & 5 & 0.152 & 80 \\ 
 origin &  D1+1 40 & 1 & True & 2 & 5 & 0.16 & 80 \\ 
 CMA 0 &  CMA 10 & 1 & True & 3 & 111 & 0.507 & 101 \\ 
 CMA 0 &  CMA 10 & 1 & True & 3 & 5 & 0.095 & 97 \\ 
 CMA 0 &  CMA 20 & 1 & True & 3 & 111 & 0.622 & 100 \\ 
 CMA 0 &  CMA 20 & 1 & True & 3 & 5 & 0.132 & 97 \\ 
 CMA 0 &  CMA 40 & 1 & True & 3 & 111 & 0.729 & 98 \\ 
 CMA 0 &  CMA 40 & 1 & True & 3 & 5 & 0.174 & 88 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 3 & 111 & 0.09 & 102 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 3 & 5 & 0.012 & 83 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 3 & 111 & 0.146 & 100 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 3 & 5 & 0.021 & 38 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 3 & 111 & 0.232 & 91 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 3 & 5 & 0.029 & 41 \\ 
 origin &  CMA 10 & 1 & True & 3 & 5 & 0.231 & 63 \\ 
\end{tabular}
\begin{tabular}{|c|c|c|c|c|c|c|c|}\\  Source & Target & Num. vars & Related side & Arity & Variable & Before fix & After fix (%
  CMA 0 &  CMA 10 & 80 & True & 2 & 111 & 0.507 & 86 \\ 
 CMA 0 &  CMA 10 & 80 & True & 2 & 5 & 0.095 & 24 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 111 & 0.622 & 84 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 5 & 0.132 & 28 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 111 & 0.729 & 82 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 5 & 0.174 & 32 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 111 & 0.09 & 97 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 5 & 0.012 & 16 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 111 & 0.146 & 88 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 5 & 0.021 & 42 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 111 & 0.232 & 93 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 5 & 0.029 & 41 \\ 
 origin &  CMA 10 & 80 & True & 2 & 5 & 0.231 & 29 \\ 
 origin &  CMA 20 & 80 & True & 2 & 5 & 0.273 & 33 \\ 
 origin &  CMA 40 & 80 & True & 2 & 5 & 0.321 & 40 \\ 
 origin &  D1+1 10 & 80 & True & 2 & 5 & 0.142 & 30 \\ 
 origin &  D1+1 20 & 80 & True & 2 & 5 & 0.152 & 32 \\ 
 origin &  D1+1 40 & 80 & True & 2 & 5 & 0.16 & 26 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 111 & 0.507 & 99 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 5 & 0.095 & 92 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 111 & 0.622 & 100 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 5 & 0.132 & 97 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 111 & 0.729 & 99 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 5 & 0.174 & 100 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 2 & 111 & 0.09 & 128 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 2 & 5 & 0.012 & 41 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 2 & 111 & 0.146 & 98 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 2 & 5 & 0.021 & 90 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 2 & 111 & 0.232 & 98 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 2 & 5 & 0.029 & 17 \\ 
 origin &  CMA 10 & 1 & True & 2 & 5 & 0.231 & 53 \\ 
 origin &  CMA 20 & 1 & True & 2 & 5 & 0.273 & 53 \\ 
 origin &  CMA 40 & 1 & True & 2 & 5 & 0.321 & 67 \\ 
 origin &  D1+1 10 & 1 & True & 2 & 5 & 0.142 & 80 \\ 
 origin &  D1+1 20 & 1 & True & 2 & 5 & 0.152 & 80 \\ 
 origin &  D1+1 40 & 1 & True & 2 & 5 & 0.16 & 80 \\ 
 CMA 0 &  CMA 10 & 1 & True & 3 & 111 & 0.507 & 101 \\ 
 CMA 0 &  CMA 10 & 1 & True & 3 & 5 & 0.095 & 97 \\ 
 CMA 0 &  CMA 20 & 1 & True & 3 & 111 & 0.622 & 100 \\ 
 CMA 0 &  CMA 20 & 1 & True & 3 & 5 & 0.132 & 97 \\ 
 CMA 0 &  CMA 40 & 1 & True & 3 & 111 & 0.729 & 98 \\ 
 CMA 0 &  CMA 40 & 1 & True & 3 & 5 & 0.174 & 88 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 3 & 111 & 0.09 & 102 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 3 & 5 & 0.012 & 83 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 3 & 111 & 0.146 & 100 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 3 & 5 & 0.021 & 38 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 3 & 111 & 0.232 & 91 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 3 & 5 & 0.029 & 41 \\ 
 origin &  CMA 10 & 1 & True & 3 & 5 & 0.231 & 63 \\ 
 origin &  CMA 20 & 1 & True & 3 & 5 & 0.273 & 24 \\ 
\end{tabular}
\begin{tabular}{|c|c|c|c|c|c|c|c|}\\  Source & Target & Num. vars & Related side & Arity & Variable & Before fix & After fix (%
  CMA 0 &  CMA 10 & 80 & True & 2 & 111 & 0.507 & 86 \\ 
 CMA 0 &  CMA 10 & 80 & True & 2 & 5 & 0.095 & 24 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 111 & 0.622 & 84 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 5 & 0.132 & 28 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 111 & 0.729 & 82 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 5 & 0.174 & 32 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 111 & 0.09 & 97 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 5 & 0.012 & 16 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 111 & 0.146 & 88 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 5 & 0.021 & 42 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 111 & 0.232 & 93 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 5 & 0.029 & 41 \\ 
 origin &  CMA 10 & 80 & True & 2 & 5 & 0.231 & 29 \\ 
 origin &  CMA 20 & 80 & True & 2 & 5 & 0.273 & 33 \\ 
 origin &  CMA 40 & 80 & True & 2 & 5 & 0.321 & 40 \\ 
 origin &  D1+1 10 & 80 & True & 2 & 5 & 0.142 & 30 \\ 
 origin &  D1+1 20 & 80 & True & 2 & 5 & 0.152 & 32 \\ 
 origin &  D1+1 40 & 80 & True & 2 & 5 & 0.16 & 26 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 111 & 0.507 & 99 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 5 & 0.095 & 92 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 111 & 0.622 & 100 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 5 & 0.132 & 97 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 111 & 0.729 & 99 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 5 & 0.174 & 100 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 2 & 111 & 0.09 & 128 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 2 & 5 & 0.012 & 41 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 2 & 111 & 0.146 & 98 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 2 & 5 & 0.021 & 90 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 2 & 111 & 0.232 & 98 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 2 & 5 & 0.029 & 17 \\ 
 origin &  CMA 10 & 1 & True & 2 & 5 & 0.231 & 53 \\ 
 origin &  CMA 20 & 1 & True & 2 & 5 & 0.273 & 53 \\ 
 origin &  CMA 40 & 1 & True & 2 & 5 & 0.321 & 67 \\ 
 origin &  D1+1 10 & 1 & True & 2 & 5 & 0.142 & 80 \\ 
 origin &  D1+1 20 & 1 & True & 2 & 5 & 0.152 & 80 \\ 
 origin &  D1+1 40 & 1 & True & 2 & 5 & 0.16 & 80 \\ 
 CMA 0 &  CMA 10 & 1 & True & 3 & 111 & 0.507 & 101 \\ 
 CMA 0 &  CMA 10 & 1 & True & 3 & 5 & 0.095 & 97 \\ 
 CMA 0 &  CMA 20 & 1 & True & 3 & 111 & 0.622 & 100 \\ 
 CMA 0 &  CMA 20 & 1 & True & 3 & 5 & 0.132 & 97 \\ 
 CMA 0 &  CMA 40 & 1 & True & 3 & 111 & 0.729 & 98 \\ 
 CMA 0 &  CMA 40 & 1 & True & 3 & 5 & 0.174 & 88 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 3 & 111 & 0.09 & 102 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 3 & 5 & 0.012 & 83 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 3 & 111 & 0.146 & 100 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 3 & 5 & 0.021 & 38 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 3 & 111 & 0.232 & 91 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 3 & 5 & 0.029 & 41 \\ 
 origin &  CMA 10 & 1 & True & 3 & 5 & 0.231 & 63 \\ 
 origin &  CMA 20 & 1 & True & 3 & 5 & 0.273 & 24 \\ 
 origin &  CMA 40 & 1 & True & 3 & 5 & 0.321 & 64 \\ 
\end{tabular}
\begin{tabular}{|c|c|c|c|c|c|c|c|}\\  Source & Target & Num. vars & Related side & Arity & Variable & Before fix & After fix (%
  CMA 0 &  CMA 10 & 80 & True & 2 & 111 & 0.507 & 86 \\ 
 CMA 0 &  CMA 10 & 80 & True & 2 & 5 & 0.095 & 24 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 111 & 0.622 & 84 \\ 
 CMA 0 &  CMA 20 & 80 & True & 2 & 5 & 0.132 & 28 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 111 & 0.729 & 82 \\ 
 CMA 0 &  CMA 40 & 80 & True & 2 & 5 & 0.174 & 32 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 111 & 0.09 & 97 \\ 
 D1+1 0 &  D1+1 10 & 80 & True & 2 & 5 & 0.012 & 16 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 111 & 0.146 & 88 \\ 
 D1+1 0 &  D1+1 20 & 80 & True & 2 & 5 & 0.021 & 42 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 111 & 0.232 & 93 \\ 
 D1+1 0 &  D1+1 40 & 80 & True & 2 & 5 & 0.029 & 41 \\ 
 origin &  CMA 10 & 80 & True & 2 & 5 & 0.231 & 29 \\ 
 origin &  CMA 20 & 80 & True & 2 & 5 & 0.273 & 33 \\ 
 origin &  CMA 40 & 80 & True & 2 & 5 & 0.321 & 40 \\ 
 origin &  D1+1 10 & 80 & True & 2 & 5 & 0.142 & 30 \\ 
 origin &  D1+1 20 & 80 & True & 2 & 5 & 0.152 & 32 \\ 
 origin &  D1+1 40 & 80 & True & 2 & 5 & 0.16 & 26 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 111 & 0.507 & 99 \\ 
 CMA 0 &  CMA 10 & 1 & True & 2 & 5 & 0.095 & 92 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 111 & 0.622 & 100 \\ 
 CMA 0 &  CMA 20 & 1 & True & 2 & 5 & 0.132 & 97 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 111 & 0.729 & 99 \\ 
 CMA 0 &  CMA 40 & 1 & True & 2 & 5 & 0.174 & 100 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 2 & 111 & 0.09 & 128 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 2 & 5 & 0.012 & 41 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 2 & 111 & 0.146 & 98 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 2 & 5 & 0.021 & 90 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 2 & 111 & 0.232 & 98 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 2 & 5 & 0.029 & 17 \\ 
 origin &  CMA 10 & 1 & True & 2 & 5 & 0.231 & 53 \\ 
 origin &  CMA 20 & 1 & True & 2 & 5 & 0.273 & 53 \\ 
 origin &  CMA 40 & 1 & True & 2 & 5 & 0.321 & 67 \\ 
 origin &  D1+1 10 & 1 & True & 2 & 5 & 0.142 & 80 \\ 
 origin &  D1+1 20 & 1 & True & 2 & 5 & 0.152 & 80 \\ 
 origin &  D1+1 40 & 1 & True & 2 & 5 & 0.16 & 80 \\ 
 CMA 0 &  CMA 10 & 1 & True & 3 & 111 & 0.507 & 101 \\ 
 CMA 0 &  CMA 10 & 1 & True & 3 & 5 & 0.095 & 97 \\ 
 CMA 0 &  CMA 20 & 1 & True & 3 & 111 & 0.622 & 100 \\ 
 CMA 0 &  CMA 20 & 1 & True & 3 & 5 & 0.132 & 97 \\ 
 CMA 0 &  CMA 40 & 1 & True & 3 & 111 & 0.729 & 98 \\ 
 CMA 0 &  CMA 40 & 1 & True & 3 & 5 & 0.174 & 88 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 3 & 111 & 0.09 & 102 \\ 
 D1+1 0 &  D1+1 10 & 1 & True & 3 & 5 & 0.012 & 83 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 3 & 111 & 0.146 & 100 \\ 
 D1+1 0 &  D1+1 20 & 1 & True & 3 & 5 & 0.021 & 38 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 3 & 111 & 0.232 & 91 \\ 
 D1+1 0 &  D1+1 40 & 1 & True & 3 & 5 & 0.029 & 41 \\ 
 origin &  CMA 10 & 1 & True & 3 & 5 & 0.231 & 63 \\ 
 origin &  CMA 20 & 1 & True & 3 & 5 & 0.273 & 24 \\ 
 origin &  CMA 40 & 1 & True & 3 & 5 & 0.321 & 64 \\ 
 origin &  D1+1 10 & 1 & True & 3 & 5 & 0.142 & 79 \\ 
\end{tabular}

